A new look at the infrared properties of z $\sim$ 5 galaxies

Recent ALMA large surveys unveiled the presence of significant dust continuum emission in star-forming galaxies at $z>4$. Unfortunately, such large programs -- i.e. ALPINE ($z\sim 5$) and REBELS ($z \sim 7$) -- only provide us with a single Far-Infrared (FIR) continuum data point for their individual targets. Therefore, high-$z$ galaxies FIR spectral energy densities (SEDs) remain mostly unconstrained, hinging on an assumption for their dust temperature ($T_{\rm d}$) in the SED fitting procedure. This introduces uncertainties in the inferred dust masses ($M_{\rm d }$), infrared luminosities ($L_{\rm IR}$), and obscured Star Formation Rate (SFR) fraction at $z > 4$. In this work we use a method that allows us to constrain $T_{\rm d}$ with a single band measurement by combining the $158\ \mathrm{\mu m}$ continuum information with the overlying [CII] emission line. We analyse the $21$ [CII] and FIR continuum detected $z\sim 5$ galaxies in ALPINE, finding a range of $T_{\rm d}=25-60\ \mathrm{K}$ and $M_{\rm d} = 0.6-25.1\ \times 10^{7}\ \mathrm{M_{\odot}}$. Given the measured stellar masses of ALPINE galaxies, the inferred dust yields are around $M_{\rm d}/M_{\star} = (0.2-8) \times 10^{-3}$, consistent with theoretical dust-production constraints. We find that $8$ out of $21$ ALPINE galaxies have $L_{\rm IR} \geq 10^{12}\ \mathrm{L_{\odot}}$, comparable to UltraLuminous IR Galaxies (ULIRGs). Relying on ultraviolet-to-optical SED fitting, the SFR was underestimated by up to $2$ orders of magnitude in $4$ of these $8$ ULIRGs-like galaxies. We conclude that these $4$ peculiar sources should be characterised by a two-phase interstellar medium structure with "spatially-segregated" FIR and ultraviolet emitting regions.

==> additional_tex_files/hyperlink_hack.tex <==

%-----------------------------------------
% avoids the 
%   \pdfendlink ended up in different nesting level than \pdfstartlink.\AtBegShi@Output ...ipout \box \AtBeginShipoutBox
% error
%-----------------------------------------
%
% see https://tex.stackexchange.com/questions/249579/pdfendlink-ended-up-in-different-nesting-level-than-pdfstartlink-error-with

% different workaround
%\AtBeginShipout{%
%  \ifnum\value{page}>1 %
%    \typeout{* Additional boxing of page `\thepage'}%
%    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
%  \fi
%}

\usepackage{etoolbox}
\makeatletter
\newcount\c@additionalboxlevel
\setcounter{additionalboxlevel}{0}
\newcount\c@maxboxlevel
\setcounter{maxboxlevel}{1}
\patchcmd\@combinedblfloats{\box\@outputbox}{%
  \stepcounter{additionalboxlevel}%
  \box\@outputbox
}{}{\errmessage{\noexpand\@combinedblfloats could not be patched}}

\AtBeginShipout{%
  \ifnum\value{additionalboxlevel}>\value{maxboxlevel}%
    \typeout{Warning: maxboxlevel might be too small, increase to %
      \the\value{additionalboxlevel}%
    }%
  \fi 
  \@whilenum\value{additionalboxlevel}<\value{maxboxlevel}\do{%
    \typeout{* Additional boxing of page `\thepage'}%
    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
    \stepcounter{additionalboxlevel}%
  }%
  \setcounter{additionalboxlevel}{0}%
}
\makeatother


==> dust properties z=5/additional_tex_files/def.tex <==


\newcommand{\skippage}[0]{\null\thispagestyle{empty}\clearpage}
\newcommand{\quotes}[1]{``#1''}
\newcommand\code[1]{\textsc{\MakeLowercase{#1}}}

% units
\def\mum{\mu{\rm m}}
\newcommand{\angstrom}{\textup{\AA}}
\def\pk{{\rm erg\,cm}^{-3}\,{\rm K}}
\def\skms{\sigma_{\rm kms}}
\def\tmyr{t_{\rm Myr}}
% constants
\def\zsun{{\rm Z}_{\odot}}
\def\msun{{\rm M}_{\odot}}
\def\lsun{{\rm L}_{\odot}}
% variables
\def\TdL{\langle T_d \rangle_L}
\def\TdM{\langle T_d \rangle_M}
\def\Tda{\langle T_d \rangle_a}
\def\SFR{\rm SFR}


% math
\def\gtsima{$\; \buildrel > \over \sim \;$}
\def\ltsima{$\; \buildrel < \over \sim \;$}
\def\gsim{\lower.5ex\hbox{\gtsima}}
\def\lsim{\lower.5ex\hbox{\ltsima}}
\def\gtsima{$\; \buildrel > \over \sim \;$} 
\def\ltsima{$\; \buildrel < \over \sim \;$} \def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\simgt{\lower.5ex\hbox{\gtsima}} 
\def\simlt{\lower.5ex\hbox{\ltsima}} 

%\def\gtsima{$\; \buildrel > \over \sim \;$} 
%\def\ltsima{$\; \buildrel < \over \sim \;$}
%\def\gsim{\lower.5ex\hbox{\gtsima}} 
%\def\lsim{\lower.5ex\hbox{\ltsima}} 

\def\be{\begin{equation}}
\def\ee{\end{equation}}

\def\NII{\hbox{[N~$\scriptstyle\rm II $]}}
\def\HII{\hbox{H~$\scriptstyle\rm II $~}}
\def\HI{\hbox{H~$\scriptstyle\rm I $~}}
\def\Hb{\hbox{H$\beta $~}}
\def\Ha{\hbox{H$\alpha $~}}
\def\OI{\hbox{[O~$\scriptstyle\rm I $]}}
\def\OII{\hbox{[O~$\scriptstyle\rm II $]}}
\def\CII{\hbox{[C~$\scriptstyle\rm II $]}}
\def\HI{\hbox{H~$\scriptstyle\rm I\ $}} 
\def\HII{\hbox{H~$\scriptstyle\rm II\ $}} 
\def\HeI{\hbox{He~$\scriptstyle\rm I\ $}} 
\def\HeII{\hbox{He~$\scriptstyle\rm II\ $}}
\def\NIII{\hbox{[N~$\scriptstyle\rm III $]}}
\def\OIII{\hbox{[O~$\scriptstyle\rm III $]}}
\def\CIII{\hbox{C~$\scriptstyle\rm III $]}} 
\def\SCII{\Sigma_{\rm [CII]}}
\def\SOIII{\Sigma_{\rm [OIII]}}
\def\SNII{\Sigma_{\rm [NII]}}
\def\SigmaCII{\Sigma_{\rm C+}}
\def\SigmaOIII{\Sigma_{\rm O++}}
\def\SigmaNII{\Sigma_{\rm N+}}
\def\HeIII{\hbox{He~$\scriptstyle\rm III\ $}} 
\def\CIV{\hbox{C~$\scriptstyle\rm IV\ $}} 
\def\SIV{\hbox{Si~$\scriptstyle\rm IV\ $}} 
\def\OVI{\hbox{O~$\scriptstyle\rm VI\ $}} \def\nHI{{\rm HI}} 
\def\nCIV{{\rm CIV}} \def\nOVI{{\rm OVI}} \def\nH{{\rm H}} 
\def\nHII{{\rm HII}} \def\nHe{{\rm He}} \def\nHeI{{\rm HeI}} 
\def\nHeII{{\rm HeII}} \def\nHeIII{{\rm HeIII}} 

%\providecommand{\angstrom}{\ensuremath{\mbox{\AA}}} % this makes a poor rendering in subscripts



==> dust properties z=5/additional_tex_files/hyperlink_hack.tex <==

%-----------------------------------------
% avoids the 
%   \pdfendlink ended up in different nesting level than \pdfstartlink.\AtBegShi@Output ...ipout \box \AtBeginShipoutBox
% error
%-----------------------------------------
%
% see https://tex.stackexchange.com/questions/249579/pdfendlink-ended-up-in-different-nesting-level-than-pdfstartlink-error-with

% different workaround
%\AtBeginShipout{%
%  \ifnum\value{page}>1 %
%    \typeout{* Additional boxing of page `\thepage'}%
%    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
%  \fi
%}

\usepackage{etoolbox}
\makeatletter
\newcount\c@additionalboxlevel
\setcounter{additionalboxlevel}{0}
\newcount\c@maxboxlevel
\setcounter{maxboxlevel}{1}
\patchcmd\@combinedblfloats{\box\@outputbox}{%
  \stepcounter{additionalboxlevel}%
  \box\@outputbox
}{}{\errmessage{\noexpand\@combinedblfloats could not be patched}}

\AtBeginShipout{%
  \ifnum\value{additionalboxlevel}>\value{maxboxlevel}%
    \typeout{Warning: maxboxlevel might be too small, increase to %
      \the\value{additionalboxlevel}%
    }%
  \fi 
  \@whilenum\value{additionalboxlevel}<\value{maxboxlevel}\do{%
    \typeout{* Additional boxing of page `\thepage'}%
    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
    \stepcounter{additionalboxlevel}%
  }%
  \setcounter{additionalboxlevel}{0}%
}
\makeatother


==> dust properties z=5/additional_tex_files/journals.tex <==

\def\amp{\&}
\def\nat{Nature}
\def\na{New Astronomy}
\def\pra{Phys. Rev. A}
\def\prb{Phys. Rev. B}
\def\prc{Phys. Rev. B}
\def\prd{Phys. Rev. D}
\def\mnras{MNRAS}
\def\apj{ApJ}
\def\apjl{ApJL}
\def\apjs{ApJS}
\def\aap{A\&A}
\def\aaps{A\&A Supp.}
\def\aapr{A\&A Rev.}
\def\araa{ARA\&A}
\def\aj{AJ}
\def\qjras{QJRAS}
\def\physrep{Phys. Rep.}
\def\apss{Ap\&SS}               % Astrophysics and Space Science
\def\planss{P\&SS}              % Planetary and Space Science
\def\pasa{Publ. Astr. Soc. Australia}
\def\pasp{Publ. Astr. Soc. Pac.}
\def\jcp{J. Chem. Phys.}
\def\pasj{Pub. Astron. Soc. Japan}
\def\ssr{Space Science Reviews}
\def\grl{Geophysical Research Letters}
\def\jgr{Journal of Geophysical Research}
\def\nar{New Astronomy Reviews}
\def\jcap{JCAP}
\def\fcp{Fundamentals of Cosmic Physics}


==> dust properties z=5/additional_tex_files/package.tex <==

\usepackage{txfonts}
\usepackage[T1]{fontenc}
\usepackage{ae,aecompl}

\usepackage{graphicx}

% to avoid conflict let amsmath redefine some stuff
\let\iiint=\relax
\let\iiiint=\relax
\let\idotsint=\relax
\let\iint=\relax
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}

\usepackage{xcolor}

\usepackage{breakcites}
\usepackage{hyperref}
\usepackage{footnote}

\usepackage{comment}

\usepackage{xfrac}
